A high fidelity synthetic face framework for computer vision

Analysis of faces is one of the core applications of computer vision, with tasks ranging from landmark alignment, head pose estimation, expression recognition, and face recognition among others. However, building reliable methods requires time-consuming data collection and often even more time-consuming manual annotation, which can be unreliable. In our work we propose synthesizing such facial data, including ground truth annotations that would be almost impossible to acquire through manual annotation at the consistency and scale possible through use of synthetic data. We use a parametric face model together with hand crafted assets which enable us to generate training data with unprecedented quality and diversity (varying shape, texture, expression, pose, lighting, and hair).

==> experiments.tex <==
Comparing on two face related tasks for which annotation labels are really difficult to acquire: head pose and dense UVs.

\subsection{Head Pose}

\subsection{UVs}

Compare to 3DDFA \cite{Zhu2017}

\emph{Describe our data-driven model.} \\
Network architecture, training, losses, \dots


\subsection{Comparison to State-of-the-Art Methods}
\emph{Basic prove for the validity of the employed baseline (approach/method).} \\
Compare to other methods on the same data/tasks they have been tested on in their papers.
Only test on sparse landmarks here since this is the common task on which all other methods 
tested their approaches (at least) and should be enough to prove the basic validity.
See Tab.~\ref{tab:sotamethods}.

% \noindent Experiments:
% \begin{itemize}
%  \item ours trained on synth. vs. results from 
%  papers~\cite{Guller2017,Yu2017}, 
%  i.e., test on datasets in papers: 
%  AFLW2000-3D (used in~\cite{Yu2017}),
%  300W challenge test set (used in~\cite{Guller2017}).
% \end{itemize}

\begin{table}[ht]
\caption{
  \textbf{Comparison to dense landmark estimation state-of-the-art methods.} 
  Comparison to the approach of Yu et al.~\cite{Yu2017} 
  on AFLW2000-3D (Note: no public code or data from Yu et al.; 
  quantitatively they evaluated on sparse landmark detection on different AFLW-based datasets, 
  incl. AFLW2000-3D (68 landmarks);
  for AFLW2000-3D they compared on different yaw angle ranges ([0,30], [30,60], [60,90]) 
  separately on all landmarks and on visible inner landmarks; Yu et al. used NMS metric; 
  Fang et al.~\cite{Feng2018} 
  evaluated on all AFLW2000-3D landmarks with the same yaw angle range split;
  G{\"u}ler et al. used AUC and failure rate (and plots of cumulative error))
}
\begin{center}
\begin{tabular}{l S[table-format=2.2] S[table-format=2.2]}
\toprule
Method & {AFLW(2000-3D)} & {300W test set} \\ 
\midrule
Yu et al.~\cite{Yu2017} 
  {\color{gray_ours}(from paper; synth \& 300W-LP)} & 3.58 & {-} \\
G{\"u}ler et al.~\cite{Guller2017} 
  {\color{gray_ours}(from paper; $\sim$3k from 300W-LP)} & {-} & 10.83 \\
Feng et al.~\cite{Feng2018} 
  {\color{gray_ours}(from paper; 300W-LP)} & {-} & {-} \\
Synth {\color{gray_ours}(our baseline; our synth)} & {TODOs~\ref{sec:todos:vsmethodyu}} & {TODOs~\ref{sec:todos:vsmethodguler}} \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:sotamethods}
\end{table}

\TODO{We probably also want to do this basic prove of the validity of the model for other tasks 
(we are evaluating on later).}


\subsection{Comparison to State-of-the-Art Datasets}
\emph{Prove the effectiveness of the proposed dataset.} \\
Compare to the same method (our baseline) when trained on datasets, 
which have been used before for this task.
Evaluate for different tasks here: (i) UV, (ii) semantic segmentation 
(at least eval for this; can best show one of the advantages of dense labeling: 
any labeling on template can be transfered to image), \dots
See Tab.~\ref{tab:sotadata}.

% \noindent Experiments:
% \begin{itemize}
%  \item baseline method(s) (e.g., UNet) trained on our synth. data vs. trained on datasets 
%  used in papers; \\
%  Compare to train sets:
%  (i) synth. data + 300W-LP + 300W challenge test set 
%  (used in~\cite{Yu2017}),
%  (ii) $\sim$3k images from 300W-LP (used in~\cite{Guller2017}); \\
%  test on 
%  (i) our real dataset (scans), 
%  (ii) our synth. test set, 
%  (iii) qualitative,
%  (iv) other (e.g., their) test sets?, \dots.
% \end{itemize}


\begin{table}[ht]
\caption{
  \textbf{Comparison to dense landmark estimation datasets.} 
  Same model architecture, different datasets
  (Probably no need to compare to data from G{\"u}ler et al.~\cite{Guller2017} 
  as their data is a subset of the data from Yu et al. -- 
  as long as we transform the data from Yu to UV annotations instead of their 2D flows)
  }
\begin{center}
\begin{tabular}{l S[table-format=2.2] S[table-format=2.2] S[table-format=2.2] S[table-format=2.2]}
\toprule
 & \multicolumn{2}{c}{Synth} & \multicolumn{2}{c}{Real (IR scans)} \\
 & {UV} & {sem. seg.} & {UV} & {sem. seg.} \\  
\midrule
Synth from Yu et al.~\cite{Yu2017} 
  & {TODOs~\ref{sec:todos:vsdatayu_onuv}} & {TODOs~\ref{sec:todos:vsdatayu_onsemseg}} & {TODOs~\ref{sec:todos:vsdatayu_onuv}} & {TODOs~\ref{sec:todos:vsdatayu_onsemseg}} \\
Real from Yu et al.~\cite{Yu2017} 
  (superset of~\cite{Guller2017})
  & {TODOs~\ref{sec:todos:vsdatayu_onuv}} & {TODOs~\ref{sec:todos:vsdatayu_onsemseg}} & {TODOs~\ref{sec:todos:vsdatayu_onuv}} & {TODOs~\ref{sec:todos:vsdatayu_onsemseg}} \\
All data from Yu et al.~\cite{Yu2017} 
  & {TODOs~\ref{sec:todos:vsdatayu_onuv}} & {TODOs~\ref{sec:todos:vsdatayu_onsemseg}} & {TODOs~\ref{sec:todos:vsdatayu_onuv}} & {TODOs~\ref{sec:todos:vsdatayu_onsemseg}} \\
Our synth & {TODOs~\ref{sec:todos:vsdataours_onuv}} & {TODOs~\ref{sec:todos:vsdataours_onsemseg}} & {TODOs~\ref{sec:todos:vsdataours_onuv}} & {TODOs~\ref{sec:todos:vsdataours_onsemseg}} \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:sotadata}
\end{table}



\subsection{Effect of Dataset Size}
\emph{Evaluate effect of changing the number of training samples.} \\
(Synth. data scalable; 
but results probably still level-off more ``quickly'' (compared to other tasks) 
i.a., due to accurate and dense supervision;
hence, smaller number of samples required than for traditional datasets/tasks.)

% \noindent Experiments:
% \begin{itemize}
%  \item train baseline with different numbers of synth. samples, test on our real data (scans)
%  (if possible, do the same experiment with training of real data 
%  e.g. from 300W-LP as in~\cite{Yu2017};
%  expected to show a different behavior, i.e., less accurate for a smaller number of samples, 
%  improving stronger only with a significant amount of data and leveling off later)
% \end{itemize}

\begin{table}[ht]
\caption{
  \textbf{Effect of Dataset Size.} 
  Given the size $N$ of a data set we can publish, 
  evaluate the effect on the results of having less/more data.
  Evaluate on dense landmark estimation (Maybe have a plot here)
  }
\begin{center}
\begin{tabular}{l S[table-format=2.2] S[table-format=2.2] S[table-format=2.2] S[table-format=2.2]}
\toprule
Dataset size & {$0.01 N$} & {$0.1 N$} & {$N$} & {$10N$} \\  
\midrule
{\color{gray_ours}Synth from Yu et al.~\cite{Yu2017} }
  & \multicolumn{4}{c}{TODOs~\ref{sec:todos:datasetsizeyu_onuv}} \\
{\color{gray_ours}Real from Yu et al.~\cite{Yu2017} 
  (superset of~\cite{Guller2017}) }
  & \multicolumn{4}{c}{TODOs~\ref{sec:todos:datasetsizeyu_onuv}} \\
{\color{gray_ours}All data from Yu et al.~\cite{Yu2017} }
  & \multicolumn{4}{c}{TODOs~\ref{sec:todos:datasetsizeyu_onuv}} \\
Our synth & \multicolumn{4}{c}{TODOs~\ref{sec:todos:datasetsizeours_onuv}} \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:datasizeeffect}
\end{table}


% \subsection{TEMP: TODOs}
% For comparison on data from: 
% \begin{itemize}
%  \item Yu et al.~\cite{Yu2017}: \\
%   \textbf{train set}: get their synthetic data (not online, ask Ronald; 
%   model should be the same as in 300W-LP, 
%   i.e. Basel); to map from their annotations to our 
%   (i.e., CogFace-) UV-values for both, synthetic and real data, 
%   there are several options: \\
%   (i) fit CogFace and render UVs (as we did for scans), 
%   need to fit to each of the meshes of the public 300W-LP data and 
%   their synthetic data (can we also get meshes for those?), 
%   (for flipped samples in 300W-LP 
%   U-coords should be easily transformable (by $1-u$) after flipping),
%   probably high effort; \\
%   (ii) fit CogFace to Basel model once (e.g., to deformation free) 
%   and find corresponding/closest vertices between models, 
%   re-render the (Basel) meshes of all samples by looking up the corresponding vertices 
%   of CogFace and then the UV values in CogFace UV space, 
%   need to write/adapt custom renderer,
%   also high effort, not sure if this works well; \\
%   (iii) get their 2D flow ground truth (to frontal, mean face) 
%   and map from pixels on frontal, mean face image to our UV values (i.e., lookup), 
%   to compute the lookup we need to get the mesh for their frontal, mean face, 
%   fit CogFace to it and could then render our UV values (as we did it for the scans),
%   then their 2D flows would directly provide the lookup in the rendering of our UV values,
%   this is probably the best option but will yield low ground truth resolution 
%   for surfaces seen from an oblique angle in the frontal face image 
%   (but this can be considered an issue of their data/ground truth 
%   and we should probably anyway not try to fix it) \\
%   \textbf{test set}: only tested on landmarks, i.a., on AFLW2000-3D, 
%   the 68 landmarks are probably (partly) the same as we used, 
%   need to find the corresponding UV value for each landmark 
%   and for each prediction find the closest predicted UV value to this one 
%   (should be similar to what is done for eval in~\cite{Guller2017})
%   \item G\"uler et al.~\cite{Guller2017}: \\
%   \textbf{train set}: ask them for their ground truth annotation (not online)
%   and map from their UV-space to ours; 
%   For the mapping it's probably again best to go for option (iii) from above, 
%   but we would need to know how their UV space is defined, 
%   i.e., how it corresponds to their mesh.
%   If we get this mapping, for every UV annotation we can compute the closest position 
%   on CogFace and from that map to our UV space.
%   Otherwise, we may just fit CogFace to the meshes from some 300W-LP images 
%   (with different poses) they used,
%   render our UVs (as we did for the scans) and should get a mapping between 
%   the UV spaces for the interesting region 
%   (will need to interpolate the mapping for other images but 
%   both UV spaces seem to be smooth so that the interpolation issue is hopefully negligible).
%   (also check if the train datasets from 300W they
%   referred to in~\cite{Guller2017} 
%   contain exactly the expected/mentioned number of samples; 
%   otherwise ask R{\i}za for the exact training data); \\
%   \textbf{test set}: for landmarks tested on 300W challenge test set, 
%   this should be the same landmark definition as for AFLW2000-3D 
%   used by Yu et al.~\cite{Yu2017}, 
%   i.e., we should be able to use the same mapping between UV and keypoints;
%   for semantic segmentation its probably not that important to compare 
%   to their method, their annotation scheme, or test set, resp. 
%   (That is, we can define a mapping to semantic labels in our UV space as usual 
%   and train with their train data and test on ours 
%   (given that we mapped the UV annotations of their train data to ours))
% \end{itemize}
% 
% for evaluation of semantic segmentation: \\
% label UV space; do semantic segmentation via predicted UVs


==> introduction.tex <==
In this technical report we present our synthetic face generation pipeline.

%\noindent make clear that: 
%\TODO{
%\begin{itemize}
% \item task is important/helpful
% \item Tackles problems for which accurate data annotation is really difficutl
% \item this is the first public dataset
% \item data is of exceptional/unprecedented quality (e.g., yields good results)
%\end{itemize}
%}

% \subsection{TEMP: Arguments for the task}
% \begin{itemize}
%  \item Direct regression of model parameters has issues \\
% 	(i) non-linear relationship to output space (different for different param. groups) 
% 	$\rightarrow$ difficult to learn/optimize \\
% 	(ii) the model space might be limited
% 	(e.g., due to limited training data, limited granularity) \\
%    (Using the dense correspondences and a subsequent model fitting step 
%    can overcome those issues)
%  \item Using the dense correspondences a subsequent model fitting step 
%    does not need to rely on visibility of sparse landmarks 
%    (similar sentence in abstract of~\cite{Yu2017})
%  \item Versatility as an intermediate representation; \\
%  model fitting, semantic segmentation, re-texturing, \dots?
%  \item More supervision for model training
% \end{itemize}


% \section{Refs}
% \subsection{Works exploiting UVs for other tasks}
% Xu et al., ICCV 2019, DenseRaC: Joint 3D Pose and Shape Estimation by Dense Render-and-Compare
% \url{http://openaccess.thecvf.com/content_ICCV_2019/papers/Xu_DenseRaC_Joint_3D_Pose_and_Shape_Estimation_by_Dense_Render-and-Compare_ICCV_2019_paper.pdf}
% (estimating body pose and shape parameters (of 3D model) based on dense landmarks)



==> related_work.tex <==
There are a large number of face datasets captured over many years by the computer vision community. 
Most of these datasets target a single task (facial landmarks, head pose, attributes, face recognition etc.).
They are often very expensive and difficult to collect especially if extra equipment is required to get ground truth annotations, such as flock of bird trackers for head pose~\cite{Cascia2000}. 
Even if specialist equipment is not required for data collection, the annotation of data is expensive, time consuming, and the resulting annotations can be very noisy \TODO{samples of noisy annotations or papers, noisy head pose}.
Sometimes, to reduce manual effort semi-automatic or fully automatic approaches to annotations have also been proposed, however, they may also lead to inaccurate annotations \TODO{300W-LP sample, dense reg, 3DDFA}
Finally, collection of such datasets poses privacy and copyright concerns, as not every person or photographer in large datasets collected by crawling the web has given concent to be included as part of the dataset.

We identify three broad categories of datasets used by the community and provide a short survey of them.

\subsection{Synthetic datasets}

A common approach to generate synthetic face data is to use a 3D morphable model of a face~\cite{Gerig2017,Richardson2016}, with either vertex or image based texture~\cite{Wood2016} models to generate synthetic data by rendering the model at various poses, illuminations, and expressions. \TODO{confirm about vertex and image}

For example, Zeng et al.~\cite{Zeng2019} used the Basel face model~\cite{Gerig2017} to generate 60K image-depth pairs of different identities, under changing pose, expression, and illumination to build a model for reconstructing fine-detail face meshes. Similarly, Richardson et al.~\cite{Richardson2017} and Sela et al.~\cite{Sela2017} used a 3D morphable model constructed from the Bosphorus dataset.~\cite{Richardson2016} to generate images together with depth, PNCC and normal maps for the task of face geometry reconstruction from images. 

SynthesEyes~\cite{Wood2015} and UnityEyes~\cite{Wood2016} also use a 3D morphable model of a face (eye region), to generate training data for eye region landmark detection and eye gaze estimation. However, they only covered a small portion of the face and did not include variations in hair styles and expressions. Further, they lack in diversity (only constructed from \TODO{N} people).

Compared to our work Basel face model does not have head hair, eyes, or teeth, and texture is fairly basic, no displacement, subsurface scattering (\TODO{see figure}). FLAME \cite{Li2017} is a more complete face model, however, it does not have textures, so is unsuitable for synthetic data generation of RGB images (but may be suitable for range data). Further, most of the datasets lack in diversity of age, and ethnicity, due to being constructed from a limited pool of subjects. \TODO{Lack of diversity in Basel}. \TODO{Hao Li synthetics?}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{./figures/related_work}
    \caption{Comparison of synthetic datasets. Note how datasets generated from Basel and Bosphorus Face models, lack full head, hair, and inside of the mouth. \TODO{missing syntheseyes and ours}}
    \label{fig:related}
\end{figure}


\subsection{Semi-synthetic datasets}

Another category of face dataset using compute graphics or image editing techniques to augment 2D or 3D datasets with varying pose and illumination.

300W-LP~\cite{Zhu2017} is a semi-synthetic dataset that creates profile faces \TODO{expand}

Another form of synthetic face data that has been used in the community is rotation and relighting of static 3D scans of faces. 
For example BU-4DFE dataset was rotated and relit to train dense RGB based landmark detectors \cite{Jeni2015}. \TODO{CLM-Z as well?}
However, this approach fairly limited due to constrained identities + expression, also hair represented badly. Further, only limited relighting is possible.

\TODO{Synthetic data with occluders? Nojavani, Xiaowei?}

\subsection{Task specific real datasets}

Issues with diversity from Celeba, and FlickrHQ, \TODO{Big focus on lack of diversity of previous datasets}, an example of a more balanced dataset is FairFace~\cite{Karkkainen2019}, however, it contains only labels for facial attributes (\TODO{confirm}), making it unsuitable for a large number of tasks.

\TODO{Head pose} - BIWI, AFLW2000, BU

\TODO{Dense and sparse landmarks}
\cite{Feng2018,Yu2017}, 

\cite{Bulat2017}

\TODO{segmentation datasets}

\TODO{hair segmentation datasets}

%\subsection{TEMP: Notes (also for eval)}
%\subsubsection{Main works on dense landmark estimation for faces}
%\begin{itemize}
% \item Feng et al., ECCV 2018~\cite{Feng2018} ($\sim$104 cites)
% \item G{\"u}ler et al., CVPR 2017~\cite{Guller2017} ($\sim$90 cites)
% \item Yu et al., ICCV 2017~\cite{Yu2017} ($\sim$18 cites)
%\end{itemize}

%\subsubsection{Train/Test sets from related work}
%Yu et al.~\cite{Yu2017} 
%train on $\sim$400k synth. data (pre-train) + 300W-LP 
%(+ also 300W challenge test set);
%test on AFLW2000-3D, AFLW and AFLW-PIFA;
%AFLW2000-3D has same annotation (68 landmarks) and fitted 3DMM model as 300W-LP;
%(Since no AFLW data was contained in 300W this can probably be considered cross-dataset.?)

%G{\"u}ler et al.~\cite{Guller2017} 
%train on data from 3DDFA 
%(but they don't seem to use the full 300W-LP, but only $\sim$3k images from 
%some subsets (see paper Sec. 4.1));
%test for landmarks (sparse) on 300W challenge test set~\cite{Sagonas2013iccvw_300wchallenge}.
%(This can probably still be considered cross-dataset as the 300W challenge test set 
%was selected independently.?).
%For semantic segmentation trained on same data and tested on Helen test set.

%Feng et al.~\cite{Feng2018} 
%train on 300W-LP;
%test on AFLW2000-3D (mainly), AFLW-PIFA and Florence;
%(Since no AFLW data was contained in 300W this can probably be considered cross-dataset.?)


%The majority of existing face datasets target a particular task, such as sparse landmark detection, attribute recognition, head pose estimation, and eye gaze tracking, while our dataset generation technique allows to extract all of that information at once, further allowing for multi-task training.

% \TODO{
% \begin{table}[t]
% \caption[dummy]{
%   \textbf{Datasets used in recent (facial landmark) papers. 
%   ICCV 2017, \dots}
%   }
% \begin{center}
% \begin{tabular}{l r}
% \toprule
% Dataset & number of usages found \\ 
% 	& (non exhaustive) \\
% \midrule
% 300W & 3 \\ 
% Florence/MICC (MICC Florence 3D Faces) & 3 \\
% WFLW & 2\\
% CelebA & 1 \\
% COFW & 1 \\
% COFW-68 (same as COFW?) & 1 \\
% BU-3DFE & 1 \\
% Menpo frontal & 1 \\
% AFLW & 1 \\
% FaceWarehouse & 1 \\
% LS3D-W (AFLW2000-3D, 300W-LP-3D, 300-VW-3D) & 1 \\
% FRGC v2.0 & 1 \\
% BU-3DFE & 1 \\
% \bottomrule
% \end{tabular}
% \end{center}
% \label{tab:unsupervised}
% \end{table}
% 
% 
% refs to add:\\
% 
% approaches for estimating face model parameters directly:\\
% ---
% Jourabloo et al, ICCV 2017,
% Pose-Invariant Face Alignment with a Single CNN
% 
% Tu et al., arxiv 2019, 
% Joint 3D Face Reconstruction and Dense Face Alignment from A Single Image with 2D-Assisted Self-Supervised Learning
% (SOTA for Face Alignment on AFLW2000-3D (cf. paperswithcode))
% 
% Gilani et al., Pattern Recognition 2017
% Deep, dense and accurate 3D face correspondence for generating population specific deformable models
% 
% 
% approaches using synthetic data:\\
% ---
% Zeng et al., ICCV 2019,
% DF2Net: A Dense-Fine-Finer Network for Detailed 3D Face Reconstruction
% (only place facial/hockey mask region (including eyes but without hair and neck) on random backgrounds)
% 
% Yu et al., \cite{Yu2017}
% (only place hockey mask region (excluding even eyes, and hair and neck) on random backgrounds)
% 
% Sela et al.~\cite{Sela2017iccv_facialreconstructionusingimagetoimagetranslation}
% (only place facial/hockey mask region (including eyes but without hair and neck) on random backgrounds)
% 
% 
% }

